Hindsight Credit Assignment

We consider the problem of efficient credit assignment in reinforcement learning. In order to efficiently and meaningfully utilize new data, we propose to explicitly assign credit to past decisions based on the likelihood of them having led to the observed outcome. This approach uses new information in hindsight, rather than employing foresight. Somewhat surprisingly, we show that value functions can be rewritten through this lens, yielding a new family of algorithms. We study the properties of these algorithms, and empirically show that they successfully address important credit assignment challenges, through a set of illustrative tasks.

==> notation.tex <==
\usepackage{bbm} % here, to make sure some of the commands load ok


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}[section]
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

% =========== Fundamental Notation =============

%=== MDP ===
\renewcommand{\P}{{\cal P}} % Transition operator
\renewcommand{\S}{\mathscr{S}} % State set
\newcommand{\A}{\mathscr{A}} % Action set
\renewcommand{\r}{r} % Reward function
\newcommand{\M}{\mathscr{M}} % MDP
\newcommand{\Rew}{\mathscr{R}} % all possible rewards
\newcommand{\X}{\mathscr{X}}

% spaces
\newcommand{\Vscr}{\mathscr{Q}}
\newcommand{\Bscr}{\mathscr{B}}

\newcommand{\Act}{\A}
\newcommand{\Rmax}{\r_{\max}}

%=== RL ===
\newcommand{\V}{v}
\newcommand{\Q}{q}

\newcommand{\F}{\mathcal{F}} % History
\newcommand{\greedy}{\mathcal{G}} % \mathcal{G} \textsc{Greedy}
\newcommand{\gr}[2]{\greedy_{#1}(#2)}

% Options
\renewcommand{\O}{\mathscr{O}} % Option set
\newcommand{\I}{\mathscr{I}} % initiation set
% models
\newcommand{\Pom}{P}
\newcommand{\Ro}{R}
\newcommand{\Toc}{\T_{\O}^c}

% Operators
\newcommand{\T}{\mathcal{T}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Ppi}{{\cal P}^\pi}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\B}{{\cal B}}

% Shaping
\newcommand{\pot}{h}
\newcommand{\Op}{\T}
\newcommand{\OpH}{\mathcal{H}}
\renewcommand{\r}{r}
\newcommand{\f}{f}
\newcommand{\ft}{F_}
\newcommand{\ssymbol}{^*}
\newcommand{\expR}{r}
\newcommand{\expF}{f}

%=== Math ===
\newcommand{\E}{\mathbb{E}} % Expectation
\newcommand{\Exp}[2]{\E_{#1}\left[#2\right]}

\newcommand\defequal{\mathrel{\overset{\makebox[0pt]{\mbox{\tiny def}}}{=}}}
%\newcommand{\eqdef}{\stackrel{\rm def}{=}}

%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\1}{\mathbb{I} } % indicator with no arguments
\newcommand{\indic}[1]{\1\{#1\}} % indicator function

\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\supnorm}[1]{\left\|#1\right\|}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\infty}}

\newcommand{\cbar}{\,|\,}

\newcommand{\Var}[1]{\mathrm{Var}\left[#1\right]}
\newcommand{\Cov}{\mathrm{Cov}}

% Number sets
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Natural}{\mathbb{N}}
\newcommand{\bN}{\Natural}

% Options
\newcommand{\To}{\T_{\O}}
\newcommand{\Po}{\P_{\O}}
\newcommand{\ppi}{\p^\pi}
\newcommand{\rpi}{\r^\pi}

%=========== Editing =============
\newcommand{\todo}[1]{{\bf[#1]}}
\newcommand{\wrt}{w.r.t. }
\newcommand{\highlight}[1]{\noindent \textbf{#1}}

% =========== Short commands and Utilities  =============
\newcommand{\ra}{\rightarrow}
\newcommand{\bld}[1]{{\boldsymbol{#1}}}

\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height
  #1\par\vskip.5\baselineskip} % From Stackexchange


\newcommand{\expE}{\E}

\newcommand{\zero}{\mathbbm 0}


% === Options lpi paper ===
\newcommand{\lpi}{$\lambda$-PI}

\newcommand{\p}{\P}
%\renewcommand{\r}{\R}
\renewcommand{\v}{v}
\newcommand{\q}{q}
\newcommand{\pio}{{\pi^o}} 
\newcommand{\bo}{\beta^o}
\newcommand{\io}{\I^o}
\newcommand{\Io}{\io}
\newcommand{\ssp}{_{ss'}}


\newcommand{\gp}{\gamma_p}
\newcommand{\Gg}{{\Gamma\gamma}}
\newcommand{\Ggp}[1]{_{\O_\Gg}^{#1}}
\newcommand{\genv}{{\gamma_r}}
\newcommand{\Tg}{\T\Ggp{\mu}}
\newcommand{\Pog}{\P\Ggp{\mu}}

\newcommand{\qgG}{\q^\mu_\Gg}
\newcommand{\qg}{\q^\mu_{\genv}}
\newcommand{\qG}{\q^\mu_{\Gamma}}
\newcommand{\PGgp}{\P\Ggp{\mu}}
\newcommand{\Pg}{\P^\mu_{\O_{\genv}}}
\newcommand{\Pgp}{\P^\mu_{\O_{\gp}}}

\newcommand{\eappr}{{\cal E}_{estim}}
\newcommand{\etarg}{{\cal E}_{targ}}

\newcommand{\dmn}{{d_{\min}}}
\newcommand{\dmx}{{d_{\max}}}

\newcommand{\go}{\Gamma_{\max}}

